ESSR: An 8K@30FPS Super-Resolution Accelerator With Edge Selective Network

Deep learning-based super-resolution (SR) is challenging to implement in resource-constrained edge devices for resolutions beyond full HD due to its high computational complexity and memory bandwidth requirements. This paper introduces an 8K@30FPS SR accelerator with edge-selective dynamic input processing. Dynamic processing chooses the appropriate subnets for different patches based on simple input edge criteria, achieving a 50\% MAC reduction with only a 0.1dB PSNR decrease. The quality of reconstruction images is guaranteed and maximized its potential with \textit{resource adaptive model switching} even under resource constraints. In conjunction with hardware-specific refinements, the model size is reduced by 84\% to 51K, but with a decrease of less than 0.6dB PSNR. Additionally, to support dynamic processing with high utilization, this design incorporates a \textit{configurable group of layer mapping} that synergizes with the \textit{structure-friendly fusion block}, resulting in 77\% hardware utilization and up to 79\% reduction in feature SRAM access. The implementation, using the TSMC 28nm process, can achieve 8K@30FPS throughput at 800MHz with a gate count of 2749K, 0.2075W power consumption, and 4797Mpixels/J energy efficiency, exceeding previous work.

==> Makefile <==
TARGET=main
LATEX_BUILD_CMD=xelatex -synctex=1 -shell-escape -interaction=nonstopmode

default: build

build:
	$(LATEX_BUILD_CMD) $(TARGET).tex
	bibtex main.aux || true
	$(LATEX_BUILD_CMD) $(TARGET).tex
	$(LATEX_BUILD_CMD) $(TARGET).tex | grep 'Warning\|pages'
clean:
	rm -rf *.aux *.log *.gz *.bbl *.blg *.lof *.lot *.toc *.out


==> publications.tex <==
\begin{publications}%


\section*{Journal Papers}
\begin{spacing}{1}
\begin{enumerate}

\item {\bf \underline{Wen-Li Yang}}, Bamboo Fox, ``Carry the Free Planets Star Fleet in Three Ways," \textit{Journal of Galaxy}, vol. 9527, no. 1, pp. 22--66, 2016

\end{enumerate}
\end{spacing}


\section*{Conference Papers}
\begin{spacing}{1}
\begin{enumerate}

\item {\bf \underline{楊威利}}, 竹狐, ``如何屌打金髮小子," in \textit{International Conference of Military History}, 2016, Iserlohn, Germany

\end{enumerate}
\end{spacing}


\end{publications}
